Learning a Unified Control Policy for Safe Falling

Being able to fall safely is a necessary motor skill for humanoids performing highly dynamic tasks, such as running and jumping. We propose a new method to learn a policy that minimizes the maximal impulse during the fall. The optimization solves for both a discrete contact planning problem and a continuous optimal control problem. Once trained, the policy can compute the optimal next contacting body part (e.g. left foot, right foot, or hands), contact location and timing, and the required joint actuation. We represent the policy as a mixture of actor-critic neural network, which consists of n control policies and the corresponding value functions. Each pair of actor-critic is associated with one of the n possible contacting body parts. During execution, the policy corresponding to the highest value function will be executed while the associated body part will be the next contact with the ground. With this mixture of actor-critic architecture, the discrete contact sequence planning is solved through the selection of the best critics while the continuous control problem is solved by the optimization of actors. We show that our policy can achieve comparable, sometimes even higher, rewards than a recursive search of the action space using dynamic programming, while enjoying 50 to 400 times of speed gain during online execution.

==> background.tex <==
\section{Background: Falling Problem as Markov Decision Process}


Researchers often model dynamics of falling motions using a simple inverted pendulum with a massless telescopic rod that connects the center of mass (COM) and the center of pressure (COP) in the sagittal plane (\figref{AbsModel}).
To illustrate the falling strategies that leverage a sequence of contacts, the inverted pendulum can be further extended by appending an additional massless telescopic rod, so-called a stopper, which mimics the reactive limb motion in human falls.
When the robot makes a new contact using a stopper, it generates an immediate impulse and establishes a new inverted pendulum pivoting the tip of the stopper.
The goal of this problem is to find the optimal sequences of stoppers and associated contacts for minimizing the maximum impulse until the robot dissipates all of its momentum.
For practical issues, it is also often assumed that the robot has a limited number of preferred contact points, such as hands, feet, or knees.

Due to its recursive property, the above problem can be formulated as a standard Markov Decision Process.
The MDP state $\vc{x}$ is defined as the state of the inverted pendulum that augmented by the discrete contact point index and time variable, $\vc{x} = \{r_1,  \theta_1, \dot{r}_1, \dot{\theta}_1, c_1, t\}$.
Similarly,  the MDP action $\vc{a}$ also can be defined as the Cartesian product of the desired velocity of the rod,  the stopper configuration, and the next contact point, $\vc{a} = \{\dot{r}_1^d, r_2, \theta_2, c_2 \}$.
Without losing generality, the length of the stopper $r_2$ can be replaced by the elapse time between impacts $\Delta t$, which leads to the revised definition $\vc{a} = \{\dot{r}_1^d, \Delta t, \theta_2, c_2 \}$.
Based on the definition of the state-action transition function $\vc{x}' = \vc{f}(\vc{x}, \vc{a})$ and the reward function $r = g(\vc{x}, \vc{a})$ in the work of \cite{}, the cost-to-go function $v$ is defined as:
\begin{equation}
  \begin{aligned}
  	v(\vc{x}) = \min_{\vc{a}} \max(g(\vc{x}, \vc{a}), v(f(\vc{x}, \vc{a}))),
  \end{aligned}
\end{equation}
where the discount factor is defined as $1.0$. 

The formulated MDP problem can be efficiently solved using dynamic programming due to its monotonic nature, where the angle of the pendulum $\theta_1$ monotonically increases from zero.
The key idea of this approach is to prevent the repetitive computation by storing the calculated cost-to-go function value for the input state into the cache, and returning the cached value when similar states are given.
For more details, please refer to the work of \cite{}.
As a result, the algorithm is able to find the global optimal solution for the given discretization within a relatively short amount of time.
However, the computation of the algorithm is still far from real-time which make it hard to be applied to real-world robots. 
